TutorUp: What If Your Students Were Simulated? Training Tutors to Address Engagement Challenges in Online Learning

With the rise of online learning, many novice tutors lack experience engaging students remotely. We introduce TutorUp, a Large Language Model (LLM)-based system that enables novice tutors to practice engagement strategies with simulated students through scenario-based training. Based on a formative study involving two surveys (N1=86, N2=102) on student engagement challenges, we summarize scenarios that mimic real teaching situations. To enhance immersion and realism, we employ a prompting strategy that simulates dynamic online learning dialogues. TutorUp provides immediate and asynchronous feedback by referencing tutor-students online session dialogues and evidence-based teaching strategies from learning science literature. In a within-subject evaluation (N=16), participants rated TutorUp significantly higher than a baseline system without simulation capabilities regarding effectiveness and usability. Our findings suggest that TutorUp provides novice tutors with more effective training to learn and apply teaching strategies to address online student engagement challenges.

==> Sections/abstract.tex <==
% This abstract is deprecated

%\textbf{Abstract: }

% With the rise of online learning, many novice tutors who are often volunteers become online teachers. However, many lack experience in addressing the challenges that come with remote online tutoring, particularly the problem of keeping individual student engaged. While there are training materials that provide guidance on which teaching strategies can promote student engagement, practicing these strategies in live tutoring scenarios with real students is costly and may cause harm. In response, we introduce TutorUp, an LLM-driven system that allows tutors to practice teaching simulated disengaged students and receive feedback. The student disengagement scenarios in the TutorUp system are based on a formative study, which included surveys and interviews (N=108) exploring student engagement issues in online learning. Particularly, we use a prompt scheme that "tells the story" of online session dialogues to ensure realistic simulations. LLMs-powered personalized feedback is provided both immediately and asynchronously. In a within-subject evaluation (N=16), participants rated our system significantly higher than the baseline across various metrics. Compared to the baseline system, TutorUp allows tutors to more effectively learn and apply strategies for engaging students. \todo{Add a sentence on the wider implications of this work.}


==> tables/reactive_scenarios.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Scenario Themes. Based on tutors' descriptions of how engagement related issues surface in their classes, we simulate scenarios allowing tutors to practice teaching strategies promoting student engagement.}
\label{tab:reactiv_scenarios} % Label for referencing the table

\begin{tblr}{
  width = \linewidth,
  colspec = {Q[163]Q[437]Q[333]},
  row{1} = {c},
  cell{2}{1} = {r=5}{},
  cell{2}{2} = {r=5}{},
  cell{7}{1} = {r=3}{},
  cell{7}{2} = {r=3}{},
  cell{10}{1} = {r=2}{},
  cell{10}{2} = {r=2}{},
  hline{1-2,7,10,12-13} = {-}{},
}
Scenario Theme                  & Description                                                                                              & Reactive Scenario                                                         \\
Lack of Interest and Engagement & Students are disengaged in class, showing little interest or participation in learning activities.       & Students don't attend the class~                                          \\
                                &                                                                                                          & Students don't respond to asked questions/group messages~                 \\
                                &                                                                                                          & Students don't show reaction to the taught content (never ask questions)~ \\
                                &                                                                                                          & Students not paying attention to the lecture content                      \\
                                &                                                                                                          & Students did not want to participate                                      \\
Lack of Confidence              & Students lack confidence in their abilities, which affects their participation and performance in class. & Students not confident in themselves                                      \\
                                &                                                                                                          & Afraid to make mistakes                                                   \\
                                &                                                                                                          & Students know the answer to something but don't reply~                    \\
Varying Learning Paces          & Students appear tired and unable to concentrate, affecting their learning and engagement.                & Some students learn faster and get bored                                  \\
                                &                                                                                                          & Students making very basic errors like subtraction or multiplication      \\
Fatigue and Focus Issues        & Students appear tired and unable to concentrate, affecting their learning and engagement.                & Students appear tired in the class                                        
\end{tblr}
\end{table}
